Gaze-in-wild: A dataset for studying eye and head coordination in everyday activities

The interaction between the vestibular and ocular system has primarily been studied in controlled environments. Consequently, off-the shelf tools for categorization of gaze events (e.g. fixations, pursuits, saccade) fail when head movements are allowed. Our approach was to collect a novel, naturalistic, and multimodal dataset of eye+head movements when subjects performed everyday tasks while wearing a mobile eye tracker equipped with an inertial measurement unit and a 3D stereo camera. This Gaze-in-the-Wild dataset (GW) includes eye+head rotational velocities (deg/s), infrared eye images and scene imagery (RGB+D). A portion was labelled by coders into gaze motion events with a mutual agreement of 0.72 sample based Cohen's $\kappa$. This labelled data was used to train and evaluate two machine learning algorithms, Random Forest and a Recurrent Neural Network model, for gaze event classification. Assessment involved the application of established and novel event based performance metrics. Classifiers achieve $\sim$90$\%$ human performance in detecting fixations and saccades but fall short (60$\%$) on detecting pursuit movements. Moreover, pursuit classification is far worse in the absence of head movement information. A subsequent analysis of feature significance in our best-performing model revealed a reliance upon absolute eye and head velocity, indicating that classification does not require spatial alignment of the head and eye tracking coordinate systems. The GW dataset, trained classifiers and evaluation metrics will be made publicly available with the intention of facilitating growth in the emerging area of head-free gaze event classification.

==> References.tex <==
\begin{thebibliography}{10}
\urlstyle{rm}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\expandafter\ifx\csname doiprefix\endcsname\relax\def\doiprefix{DOI: }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{Itti1998AAnalysis}
\bibinfo{author}{Itti, L.}, \bibinfo{author}{Koch, C.} \&
  \bibinfo{author}{Niebur, E.}
\newblock \bibinfo{journal}{\bibinfo{title}{{A model of saliency-based visual
  attention for rapid scene analysis}}}.
\newblock {\emph{\JournalTitle{IEEE Transactions on Pattern Analysis and
  Machine Intelligence}}} \textbf{\bibinfo{volume}{20}},
  \bibinfo{pages}{1254--1259}, \doiprefix\url{10.1109/34.730558}
  (\bibinfo{year}{1998}).

\bibitem{Tatler2010YarbusVision}
\bibinfo{author}{Tatler, B.~W.}, \bibinfo{author}{Wade, N.~J.},
  \bibinfo{author}{Kwan, H.}, \bibinfo{author}{Findlay, J.~M.} \&
  \bibinfo{author}{Velichkovsky, B.~M.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Yarbus, eye movements, and
  vision}}}.
\newblock {\emph{\JournalTitle{i-Perception}}} \doiprefix\url{10.1068/i0382}
  (\bibinfo{year}{2010}).

\bibitem{Hayhoe2012}
\bibinfo{author}{Hayhoe, M.~M.}, \bibinfo{author}{McKinney, T.},
  \bibinfo{author}{Chajka, K.} \& \bibinfo{author}{Pelz, J.~B.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Predictive eye movements in
  natural vision}}}.
\newblock {\emph{\JournalTitle{Experimental Brain Research}}}
  \textbf{\bibinfo{volume}{217}}, \bibinfo{pages}{125--136},
  \doiprefix\url{10.1007/s00221-011-2979-2} (\bibinfo{year}{2012}).

\bibitem{Hayhoe2005EyeBehavior}
\bibinfo{author}{Hayhoe, M.} \& \bibinfo{author}{Ballard, D.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Eye movements in natural
  behavior}}}.
\newblock {\emph{\JournalTitle{Trends in Cognitive Sciences}}}
  \textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{188--194},
  \doiprefix\url{10.1016/j.tics.2005.02.009} (\bibinfo{year}{2005}).

\bibitem{Sprague2015StereopsisEnvironment}
\bibinfo{author}{Sprague, W.~W.}, \bibinfo{author}{Cooper, E.~A.},
  \bibinfo{author}{To{\v{s}}i{\'{c}}, I.} \& \bibinfo{author}{Banks, M.~S.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Stereopsis is adaptive for the
  natural environment}}}.
\newblock {\emph{\JournalTitle{Science Advances}}}
  \textbf{\bibinfo{volume}{1}}, \doiprefix\url{10.1126/sciadv.1400254}
  (\bibinfo{year}{2015}).

\bibitem{Kothari2016NovelObstacles}
\bibinfo{author}{Kothari, R.}, \bibinfo{author}{Binaee, K.},
  \bibinfo{author}{Matthis, J.~S.}, \bibinfo{author}{Bailey, R.} \&
  \bibinfo{author}{Diaz, G.~J.}
\newblock \bibinfo{title}{{Novel apparatus for investigation of eye movements
  when walking in the presence of 3D projected obstacles}}.
\newblock In \emph{\bibinfo{booktitle}{Proceedings of the Ninth Biennial ACM
  Symposium on Eye Tracking Research {\&} Applications - ETRA '16}},
  vol.~\bibinfo{volume}{14}, \bibinfo{pages}{261--266},
  \doiprefix\url{10.1145/2857491.2857540} (\bibinfo{year}{2016}).

\bibitem{Daye2014}
\bibinfo{author}{Daye, P.~M.}, \bibinfo{author}{Blohm, G.} \&
  \bibinfo{author}{Lefevre, P.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Catch-up saccades in
  head-unrestrained conditions reveal that saccade amplitude is corrected using
  an internal model of target movement}}}.
\newblock {\emph{\JournalTitle{Journal of Vision}}}
  \textbf{\bibinfo{volume}{14}}, \bibinfo{pages}{12--12},
  \doiprefix\url{10.1167/14.1.12} (\bibinfo{year}{2014}).

\bibitem{Barnes1979Vestibulo-ocularTargets.}
\bibinfo{author}{Barnes, G.~R.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Vestibulo-ocular function during
  co-ordinated head and eye movements to acquire visual targets.}}}
\newblock {\emph{\JournalTitle{The Journal of physiology}}}
  \textbf{\bibinfo{volume}{287}}, \bibinfo{pages}{127--47}
  (\bibinfo{year}{1979}).

\bibitem{Freedman2008CoordinationOrienting}
\bibinfo{author}{Freedman, E.~G.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Coordination of the eyes and head
  during visual orienting}}}.
\newblock {\emph{\JournalTitle{Experimental Brain Research}}}
  \textbf{\bibinfo{volume}{190}}, \bibinfo{pages}{369--387},
  \doiprefix\url{10.1007/s00221-008-1504-8} (\bibinfo{year}{2008}).

\bibitem{Einhauser2007}
\bibinfo{author}{Einh{\"{a}}user, W.} \emph{et~al.}
\newblock \emph{\bibinfo{title}{{Human eye-head co-ordination in natural
  exploration}}}, vol.~\bibinfo{volume}{18} (\bibinfo{publisher}{Network},
  \bibinfo{year}{2007}).

\bibitem{Matthis2018GazeTerrain}
\bibinfo{author}{Matthis, J.~S.}, \bibinfo{author}{Yates, J.~L.} \&
  \bibinfo{author}{Hayhoe, M.~M.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Gaze and the Control of Foot
  Placement When Walking in Natural Terrain}}}.
\newblock {\emph{\JournalTitle{Current Biology}}}
  \textbf{\bibinfo{volume}{28}}, \bibinfo{pages}{1224--1233},
  \doiprefix\url{10.1016/j.cub.2018.03.008} (\bibinfo{year}{2018}).

\bibitem{Epelboim1995TheTasks}
\bibinfo{author}{Epelboim, J.} \emph{et~al.}
\newblock \bibinfo{journal}{\bibinfo{title}{{The function of visual search and
  memory in sequential looking tasks}}}.
\newblock {\emph{\JournalTitle{Vision Research}}}
  \textbf{\bibinfo{volume}{35}}, \bibinfo{pages}{3401--3422},
  \doiprefix\url{10.1016/0042-6989(95)00080-X} (\bibinfo{year}{1995}).

\bibitem{fang2015eye}
\bibinfo{author}{Fang, Y.}, \bibinfo{author}{Nakashima, R.},
  \bibinfo{author}{Matsumiya, K.}, \bibinfo{author}{Kuriki, I.} \&
  \bibinfo{author}{Shioiri, S.}
\newblock \bibinfo{journal}{\bibinfo{title}{Eye-head coordination for visual
  cognitive processing}}.
\newblock {\emph{\JournalTitle{PloS one}}} \textbf{\bibinfo{volume}{10}},
  \bibinfo{pages}{e0121035} (\bibinfo{year}{2015}).

\bibitem{Allison1996CombinedSystem}
\bibinfo{author}{Allison, R.~S.}, \bibinfo{author}{Eizenman, M.} \&
  \bibinfo{author}{Cheung, B.~S.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Combined head and eye tracking
  system for dynamic testing of the vestibular system}}}.
\newblock {\emph{\JournalTitle{IEEE Transactions on Biomedical Engineering}}}
  \textbf{\bibinfo{volume}{43}}, \bibinfo{pages}{1073--1082},
  \doiprefix\url{10.1109/10.541249} (\bibinfo{year}{1996}).

\bibitem{Kinsman2012Ego-motionTracking}
\bibinfo{author}{Kinsman, T.}, \bibinfo{author}{Evans, K.},
  \bibinfo{author}{Sweeney, G.}, \bibinfo{author}{Keane, T.} \&
  \bibinfo{author}{Pelz, J.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Ego-motion compensation improves
  fixation detection in wearable eye tracking}}}.
\newblock {\emph{\JournalTitle{Proceedings of the Symposium on Eye Tracking
  Research and Applications - ETRA '12}}} \bibinfo{pages}{221},
  \doiprefix\url{10.1145/2168556.2168599} (\bibinfo{year}{2012}).

\bibitem{Larsson2016}
\bibinfo{author}{Larsson, L.}, \bibinfo{author}{Schwaller, A.},
  \bibinfo{author}{Nystr{\"{o}}m, M.} \& \bibinfo{author}{Stridh, M.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Head movement compensation and
  multi-modal event detection in eye-tracking data for unconstrained head
  movements}}}.
\newblock {\emph{\JournalTitle{Journal of Neuroscience Methods}}}
  \textbf{\bibinfo{volume}{274}}, \bibinfo{pages}{13--26},
  \doiprefix\url{10.1016/j.jneumeth.2016.09.005} (\bibinfo{year}{2016}).

\bibitem{Tomasi2016MobileStudies}
\bibinfo{author}{Tomasi, M.}, \bibinfo{author}{Pundlik, S.},
  \bibinfo{author}{Bowers, A.~R.}, \bibinfo{author}{Peli, E.} \&
  \bibinfo{author}{Luo, G.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Mobile gaze tracking system for
  outdoor walking behavioral studies}}}.
\newblock {\emph{\JournalTitle{Journal of Vision}}}
  \textbf{\bibinfo{volume}{16}}, \bibinfo{pages}{27},
  \doiprefix\url{10.1167/16.3.27} (\bibinfo{year}{2016}).

\bibitem{holmqvist2011eye}
\bibinfo{author}{Holmqvist, K.} \emph{et~al.}
\newblock \emph{\bibinfo{title}{Eye tracking: A comprehensive guide to methods
  and measures}} (\bibinfo{publisher}{OUP Oxford}, \bibinfo{year}{2011}).

\bibitem{Pekkanen2017ARegression}
\bibinfo{author}{Pekkanen, J.} \& \bibinfo{author}{Lappi, O.}
\newblock \bibinfo{journal}{\bibinfo{title}{{A new and general approach to
  signal denoising and eye movement classification based on segmented linear
  regression}}}.
\newblock {\emph{\JournalTitle{Scientific Reports}}}
  \textbf{\bibinfo{volume}{7}}, \bibinfo{pages}{1--13},
  \doiprefix\url{10.1038/s41598-017-17983-x} (\bibinfo{year}{2017}).

\bibitem{Zemblys2018UsingData}
\bibinfo{author}{Zemblys, R.}, \bibinfo{author}{Niehorster, D.~C.},
  \bibinfo{author}{Komogortsev, O.} \& \bibinfo{author}{Holmqvist, K.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Using machine learning to detect
  events in eye-tracking data}}}.
\newblock {\emph{\JournalTitle{Behavior Research Methods}}}
  \textbf{\bibinfo{volume}{50}}, \bibinfo{pages}{160--181},
  \doiprefix\url{10.3758/s13428-017-0860-3} (\bibinfo{year}{2018}).

\bibitem{Zemblys2018GazeNetNetworks}
\bibinfo{author}{Zemblys, R.}, \bibinfo{author}{Niehorster, D.~C.} \&
  \bibinfo{author}{Holmqvist, K.}
\newblock \bibinfo{journal}{\bibinfo{title}{{gazeNet : End-to-end eye-movement
  event detection with deep neural networks}}}.
\newblock }}} \doiprefix\url{10.3758/s13428-018-1133-5} (\bibinfo{year}{2018}).

\bibitem{Lappi2016EyeReference}
\bibinfo{author}{Lappi, O.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Eye movements in the wild:
  Oculomotor control, gaze behavior {\&} frames of reference}}}.
\newblock {\emph{\JournalTitle{Neuroscience and Biobehavioral Reviews}}}
  \textbf{\bibinfo{volume}{69}}, \bibinfo{pages}{49--68},
  \doiprefix\url{10.1016/j.neubiorev.2016.06.006} (\bibinfo{year}{2016}).

\bibitem{Nystrom2018IsResearchers}
\bibinfo{author}{Nystr{\"{o}}m, M.}, \bibinfo{author}{Hooge, I. T.~C.},
  \bibinfo{author}{Hessels, R.~S.}, \bibinfo{author}{Niehorster, D.~C.} \&
  \bibinfo{author}{Andersson, R.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Is the eye-movement field confused
  about fixations and saccades? A survey among 124 researchers}}}.
\newblock {\emph{\JournalTitle{Royal Society Open Science}}}
  \textbf{\bibinfo{volume}{5}}, \bibinfo{pages}{180502},
  \doiprefix\url{10.1098/rsos.180502} (\bibinfo{year}{2018}).

\bibitem{Land2009TheRepertoire}
\bibinfo{author}{Land, M.~F.} \& \bibinfo{author}{Tatler, B.~W.}
\newblock \bibinfo{title}{{The human eye movement repertoire}}.
\newblock In \emph{\bibinfo{booktitle}{Looking and ActingVision and eye
  movements in natural behaviour}}, \bibinfo{pages}{13--25},
  \doiprefix\url{10.1093/acprof:oso/9780198570943.003.0002}
  (\bibinfo{publisher}{Oxford University Press}, \bibinfo{year}{2009}).

\bibitem{Barnes1989Head-freeManner.}
\bibinfo{author}{Barnes, G.~R.} \& \bibinfo{author}{Lawson, J.~F.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Head-free pursuit in the human of
  a visual target moving in a pseudo-random manner.}}}
\newblock {\emph{\JournalTitle{The Journal of physiology}}}
  \textbf{\bibinfo{volume}{410}}, \bibinfo{pages}{137--55},
  \doiprefix\url{10.1113/jphysiol.1989.sp017525} (\bibinfo{year}{1989}).

\bibitem{Barnes1993Visual-vestibularMechanisms}
\bibinfo{author}{Barnes, G.~R.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Visual-vestibular interaction in
  the control of head and eye movement: The role of visual feedback and
  predictive mechanisms}}}.
\newblock {\emph{\JournalTitle{Progress in Neurobiology}}}
  \textbf{\bibinfo{volume}{41}}, \bibinfo{pages}{435--472},
  \doiprefix\url{10.1016/0301-0082(93)90026-O} (\bibinfo{year}{1993}).

\bibitem{A.A.Skavenski1979QualityMan}
\bibinfo{author}{{A. A. Skavenski}}, \bibinfo{author}{{R. M. Hansen}},
  \bibinfo{author}{{R. M. Steinman}} \& \bibinfo{author}{{B. J. Winterson}}.
\newblock \bibinfo{journal}{\bibinfo{title}{{Quality of retinal image
  stabilization during small natural and artificial body rotations in man}}}.
\newblock {\emph{\JournalTitle{Vision Research}}}
  \textbf{\bibinfo{volume}{19}}, \bibinfo{pages}{675--683}
  (\bibinfo{year}{1979}).

\bibitem{Martinez-Conde2004ThePerception}
\bibinfo{author}{Martinez-Conde, S.}, \bibinfo{author}{Macknik, S.~L.} \&
  \bibinfo{author}{Hubel, D.~H.}
\newblock \bibinfo{journal}{\bibinfo{title}{{The role of fixational eye
  movements in visual perception}}}.
\newblock {\emph{\JournalTitle{Nature Reviews Neuroscience}}}
  \textbf{\bibinfo{volume}{5}}, \bibinfo{pages}{229--240},
  \doiprefix\url{10.1038/nrn1348} (\bibinfo{year}{2004}).

\bibitem{Angelaki2004EyesMotion}
\bibinfo{author}{Angelaki, D.~E.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Eyes on Target: What Neurons Must
  do for the Vestibuloocular Reflex During Linear Motion}}}.
\newblock {\emph{\JournalTitle{Journal of Neurophysiology}}}
  \textbf{\bibinfo{volume}{92}}, \bibinfo{pages}{20--35},
  \doiprefix\url{10.1152/jn.00047.2004} (\bibinfo{year}{2004}).

\bibitem{Angelaki2006Three-DimensionalConstraints}
\bibinfo{author}{Angelaki, D.~E.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Three-Dimensional Ocular
  Kinematics During Eccentric Rotations: Evidence for Functional Rather Than
  Mechanical Constraints}}}.
\newblock {\emph{\JournalTitle{Journal of Neurophysiology}}}
  \doiprefix\url{10.1152/jn.01137.2002} (\bibinfo{year}{2006}).

\bibitem{mustari2010optokinetic}
\bibinfo{author}{Mustari, M.} \& \bibinfo{author}{Ono, S.}
\newblock \bibinfo{title}{Optokinetic eye movements}.
\newblock In \emph{\bibinfo{booktitle}{Encyclopedia of Neuroscience}}
  (\bibinfo{publisher}{Elsevier Ltd}, \bibinfo{year}{2010}).

\bibitem{Ackerley2011}
\bibinfo{author}{Ackerley, R.} \& \bibinfo{author}{Barnes, G.~R.}
\newblock \bibinfo{journal}{\bibinfo{title}{{The interaction of visual,
  vestibular and extra-retinal mechanisms in the control of head and gaze
  during head-free pursuit}}}.
\newblock {\emph{\JournalTitle{Journal of Physiology}}}
  \textbf{\bibinfo{volume}{589}}, \bibinfo{pages}{1627--1642},
  \doiprefix\url{10.1113/jphysiol.2010.199471} (\bibinfo{year}{2011}).

\bibitem{Matthis2014VisualTerrain}
\bibinfo{author}{Matthis, J.~S.} \& \bibinfo{author}{Fajen, B.~R.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Visual control of foot placement
  when walking over complex terrain}}}.
\newblock {\emph{\JournalTitle{Journal of Experimental Psychology: Human
  Perception and Performance}}} \doiprefix\url{10.1037/a0033101}
  (\bibinfo{year}{2014}).

\bibitem{Land2001InActivities}
\bibinfo{author}{Land, M.~F.} \& \bibinfo{author}{Hayhoe, M.}
\newblock \bibinfo{title}{{In what ways do eye movements contribute to everyday
  activities?}}
\newblock In \emph{\bibinfo{booktitle}{Vision Research}},
  \doiprefix\url{10.1016/S0042-6989(01)00102-X} (\bibinfo{year}{2001}).

\bibitem{Kassner2014Pupil:Interaction}
\bibinfo{author}{Kassner, M.}, \bibinfo{author}{Patera, W.} \&
  \bibinfo{author}{Bulling, A.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Pupil: An Open Source Platform for
  Pervasive Eye Tracking and Mobile Gaze-based Interaction}}}.
\newblock }}} \doiprefix\url{10.1145/2638728.2641695} (\bibinfo{year}{2014}).

\bibitem{i2cdevlib}
\bibinfo{author}{Rowberg, J.}
\newblock \bibinfo{title}{I2c device library}.

\bibitem{Ortiz2018DepthStereolabs}
\bibinfo{author}{Ortiz, L.~E.}, \bibinfo{author}{Cabrera, V.~E.} \&
  \bibinfo{author}{Goncalves, L. M.~G.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Depth Data Error Modeling of the
  ZED 3D Vision Sensor from Stereolabs}}}.
\newblock {\emph{\JournalTitle{ELCVIA Electronic Letters on Computer Vision and
  Image Analysis}}} \textbf{\bibinfo{volume}{17}}, \bibinfo{pages}{1--15},
  \doiprefix\url{10.5565/rev/elcvia.1084} (\bibinfo{year}{2018}).

\bibitem{Vercher1991Eye-headFixation.}
\bibinfo{author}{Vercher, J.~L.} \& \bibinfo{author}{Gauthier, G.~M.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Eye-head movement coordination:
  vestibulo-ocular reflex suppression with head-fixed target fixation.}}}
\newblock {\emph{\JournalTitle{Journal of vestibular research : equilibrium
  {\&} orientation}}} \textbf{\bibinfo{volume}{1}}, \bibinfo{pages}{161--70}
  (\bibinfo{year}{1991}).

\bibitem{Hartley:2003:MVG:861369}
\bibinfo{author}{Hartley, R.} \& \bibinfo{author}{Zisserman, A.}
\newblock \emph{\bibinfo{title}{Multiple View Geometry in Computer Vision}}
  (\bibinfo{publisher}{Cambridge University Press}, \bibinfo{address}{New York,
  NY, USA}, \bibinfo{year}{2003}), \bibinfo{edition}{2} edn.

\bibitem{Bahill1982FrequencyAlgorithm}
\bibinfo{author}{Bahill, A.~T.}, \bibinfo{author}{Kallman, J.~S.} \&
  \bibinfo{author}{Lieberman, J.~E.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Frequency limitations of the
  two-point central difference differentiation algorithm}}}.
\newblock {\emph{\JournalTitle{Biological Cybernetics}}}
  \textbf{\bibinfo{volume}{45}}, \bibinfo{pages}{1--4},
  \doiprefix\url{10.1007/BF00387207} (\bibinfo{year}{1982}).

\bibitem{Chaparro2015SignalsEdition}
\bibinfo{author}{Chaparro, L.~F.}
\newblock \emph{\bibinfo{title}{{Signals and Systems Using MATLAB: Second
  Edition}}} (\bibinfo{year}{2015}).

\bibitem{Paris2007AApplications}
\bibinfo{author}{Paris, S.}
\newblock \bibinfo{title}{{A gentle introduction to bilateral filtering and its
  applications}}.
\newblock In \emph{\bibinfo{booktitle}{ACM SIGGRAPH 2007 courses on - SIGGRAPH
  '07}}, \doiprefix\url{10.1145/1281500.1281604} (\bibinfo{year}{2007}).

\bibitem{Agtzidis2017InViewing}
\bibinfo{author}{Agtzidis, I.}, \bibinfo{author}{Startsev, M.} \&
  \bibinfo{author}{Dorr, M.}
\newblock \bibinfo{journal}{\bibinfo{title}{{In the pursuit of (ground) truth:
  A hand-labelling tool for eye movements recorded during dynamic scene
  viewing}}}.
\newblock {\emph{\JournalTitle{Proceedings of the 2nd Workshop on Eye Tracking
  and Visualization, ETVIS 2016}}} \bibinfo{pages}{65--68},
  \doiprefix\url{10.1109/ETVIS.2016.7851169} (\bibinfo{year}{2017}).

\bibitem{hooge2017human}
\bibinfo{author}{Hooge, I.~T.}, \bibinfo{author}{Niehorster, D.~C.},
  \bibinfo{author}{Nystr{\"o}m, M.}, \bibinfo{author}{Andersson, R.} \&
  \bibinfo{author}{Hessels, R.~S.}
\newblock \bibinfo{journal}{\bibinfo{title}{Is human classification by
  experienced untrained observers a gold standard in fixation detection?}}
\newblock {\emph{\JournalTitle{Behavior research methods}}}
  \bibinfo{pages}{1--18} (\bibinfo{year}{2017}).

\bibitem{Andersson2017OneAlgorithms}
\bibinfo{author}{Andersson, R.}, \bibinfo{author}{Larsson, L.},
  \bibinfo{author}{Holmqvist, K.}, \bibinfo{author}{Stridh, M.} \&
  \bibinfo{author}{Nystr{\"{o}}m, M.}
\newblock \bibinfo{journal}{\bibinfo{title}{{One algorithm to rule them all? An
  evaluation and discussion of ten eye movement event-detection algorithms}}}.
\newblock {\emph{\JournalTitle{Behavior Research Methods}}}
  \textbf{\bibinfo{volume}{49}}, \bibinfo{pages}{616--637},
  \doiprefix\url{10.3758/s13428-016-0738-9} (\bibinfo{year}{2017}).

\bibitem{Hoppe2016End-to-EndNetworks}
\bibinfo{author}{Hoppe, S.} \& \bibinfo{author}{Bulling, A.}
\newblock \bibinfo{journal}{\bibinfo{title}{{End-to-End Eye Movement Detection
  Using Convolutional Neural Networks}}}.
\newblock }}}  (\bibinfo{year}{2016}).

\bibitem{Powers2012TheKappa}
\bibinfo{author}{Powers, D. M.~W.}
\newblock \bibinfo{journal}{\bibinfo{title}{{The problem with kappa}}}.
\newblock {\emph{\JournalTitle{Conference of the European Chapter of the
  Association for Computational Linguistics}}} \bibinfo{pages}{345--355}
  (\bibinfo{year}{2012}).

\bibitem{kisler2013dialect}
\bibinfo{author}{Kisler, T.} \& \bibinfo{author}{Reichel, U.~D.}
\newblock \bibinfo{journal}{\bibinfo{title}{A dialect distance metric based on
  string and temporal alignment}}.
\newblock {\emph{\JournalTitle{Elektronische Sprachsignalverarbeitung}}}
  \bibinfo{pages}{158--165} (\bibinfo{year}{2013}).

\bibitem{Breiman1999RandomForests}
\bibinfo{author}{Breiman, L.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Random Forests}}}.
\newblock {\emph{\JournalTitle{Machine Learning}}}
  \doiprefix\url{10.1023/A:1010933404324} (\bibinfo{year}{1999}).

\bibitem{Chung2014EmpiricalModeling}
\bibinfo{author}{Chung, J.}, \bibinfo{author}{Gulcehre, C.},
  \bibinfo{author}{Cho, K.} \& \bibinfo{author}{Bengio, Y.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Empirical Evaluation of Gated
  Recurrent Neural Networks on Sequence Modeling}}}.
\newblock }}} \bibinfo{pages}{1--9}, \doiprefix\url{10.1109/IJCNN.2015.7280624}
  (\bibinfo{year}{2014}).

\bibitem{Kingma2014Adam:Optimization}
\bibinfo{author}{Kingma, D.~P.} \& \bibinfo{author}{Ba, J.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Adam: A Method for Stochastic
  Optimization}}}.
\newblock {\emph{\JournalTitle{AIP Conference Proceedings}}}
  \textbf{\bibinfo{volume}{1631}}, \bibinfo{pages}{58--62},
  \doiprefix\url{10.1016/j.jneumeth.2005.04.009} (\bibinfo{year}{2014}).

\bibitem{Karpov2013}
\bibinfo{author}{Komogortsev, O.~V.} \& \bibinfo{author}{Karpov, A.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Automated classification and
  scoring of smooth pursuit eye movements in the presence of fixations and
  saccades}}}.
\newblock {\emph{\JournalTitle{Behavior Research Methods}}}
  \textbf{\bibinfo{volume}{45}}, \bibinfo{pages}{203--215},
  \doiprefix\url{10.3758/s13428-012-0234-9} (\bibinfo{year}{2013}).

\bibitem{Santini2016}
\bibinfo{author}{Santini, T.}, \bibinfo{author}{Fuhl, W.},
  \bibinfo{author}{K{\"{u}}bler, T.} \& \bibinfo{author}{Kasneci, E.}
\newblock \bibinfo{journal}{\bibinfo{title}{{Bayesian Identification of
  Fixations, Saccades, and Smooth Pursuits}}}.
\newblock }}} \doiprefix\url{10.1145/2857491.2857512} (\bibinfo{year}{2015}).

\bibitem{Mann2013TheBall}
\bibinfo{author}{Mann, D.~L.}, \bibinfo{author}{Spratford, W.} \&
  \bibinfo{author}{Abernethy, B.}
\newblock \bibinfo{journal}{\bibinfo{title}{{The Head Tracks and Gaze Predicts:
  How the World's Best Batters Hit a Ball}}}.
\newblock {\emph{\JournalTitle{PLoS ONE}}}
  \doiprefix\url{10.1371/journal.pone.0058289} (\bibinfo{year}{2013}).

\bibitem{Daemi2015kinematicmodel}
\bibinfo{author}{Daemi, M.} \& \bibinfo{author}{Crawford, J.~D.}
\newblock \bibinfo{journal}{\bibinfo{title}{A kinematic model for 3-d head-free
  gaze-shifts}}.
\newblock {\emph{\JournalTitle{Frontiers in Computational Neuroscience}}}
  \textbf{\bibinfo{volume}{9}}, \bibinfo{pages}{1--18},
  \doiprefix\url{10.3389/fncom.2015.00072} (\bibinfo{year}{2015}).

\bibitem{morel2018gramm}
\bibinfo{author}{Morel, P.}
\newblock \bibinfo{journal}{\bibinfo{title}{Gramm: grammar of graphics plotting
  in matlab}}.
\newblock {\emph{\JournalTitle{JOSS}}} \textbf{\bibinfo{volume}{3}},
  \bibinfo{pages}{568} (\bibinfo{year}{2018}).

\end{thebibliography}

